The Role of Dust in Models of Population Synthesis

We have employed state-of-the-art evolutionary models of low and intermediate-mass AGB stars, and included the effect of circumstellar dust shells on the spectral energy distribution (SED) of AGB stars, to revise the Padua library of isochrones (Bertelli et al. 1994). The major revision involves the thermally pulsing AGB phase, that is now taken from fully evolutionary calculations by Weiss & Ferguson (2009). Two libraries of about 600 AGB dust-enshrouded SEDs each have also been calculated, one for oxygen-rich M-stars and one for carbon-rich C-stars. Each library accounts for different values of input parameters like the optical depth {\tau}, dust composition, and temperature of the inner boundary of the dust shell. These libraries of dusty AGB spectra have been implemented into a large composite library of theoretical stellar spectra, to cover all regions of the Hertzsprung-Russell Diagram (HRD) crossed by the isochrones. With the aid of the above isochrones and libraries of stellar SEDs, we have calculated the spectro-photometric properties (SEDs, magnitudes, and colours) of single-generation stellar populations (SSPs) for six metallicities, more than fifty ages (from 3 Myr to 15 Gyr), and nine choices of the Initial Mass Function. The new isochrones and SSPs have been compared to the colour-magnitude diagrams (CMDs) of field populations in the LMC and SMC, with particular emphasis on AGB stars, and the integrated colours of star clusters in the same galaxies, using data from the SAGE (Surveying the Agents of Galaxy Evolution) catalogues. We have also examined the integrated colours of a small sample of star clusters located in the outskirts of M31. The agreement between theory and observations is generally good. In particular, the new SSPs reproduce the red tails of the AGB star distribution in the CMDs of field stars in the Magellanic Clouds.

==> newcomm.tex <==
\newcommand{\BEQ}{\begin{equation}}
\newcommand{\EEQ}{\end{equation}}
%\newcommand{\barr}{\begin{array}}
%\newcommand{\earr}{\end{array}}
%\newcommand{\arry}{\begin{eqnarray}}
%\newcommand{\earry}{\end{eqnarray}}
\newcommand{\BI}{\begin{itemize}}
\newcommand{\EI}{\end{itemize}}
\newcommand{\BE}{\begin{enumerate}}
\newcommand{\EE}{\end{enumerate}}
\newcommand{\dis}{\displaystyle}
\newcommand{\BC}{\begin{center}}
\newcommand{\EC}{\end{center}}
%\newcommand{\BL}{\begin{flushleft}}
%\newcommand{\EL}{\end{flushleft}}
\newcommand{\BTA}{\begin{table}}
\newcommand{\ETA}{\end{table}}
%\newcommand{\BT}{\begin{tabbing}}
%\newcommand{\ET}{\end{tabbing}}
\newcommand{\BTAB}{\begin{tabular}}
\newcommand{\ETAB}{\end{tabular}}
\newcommand{\BD}{\begin{description}}
\newcommand{\ED}{\end{description}}
%\newcommand{\cit}{\astroncite}
%\newcommand{\la}{\lambbegin{tabbingbegin{tabbingda}
\newcommand{\BF}{\begin{figure}}
\newcommand{\EF}{\end{figure}}
%\newcommand{\acapo}{\newline \noindent}
\newcommand{\BM}{\begin{displaymath}}
\newcommand{\EM}{\end{displaymath}}
%\newcommand{\NO}{\noindent}
%\newcommand{\BL}{\begin{list}}
%\newcommand{\EL}{\end{list}}
\newcommand{\bs}{$\backslash$}
\newcommand{\mum}{$\mu m$}
\newcommand{\V}{\rule{0pt}{3.5ex}}
\newcommand{\SCP}{\shortcite}  %(lista breve, anno)
\newcommand{\SCN}{\shortciteN} %lista breve (anno) !una cit alla volta!
\newcommand{\CP}{\cite}        %(lista lunga, anno)
\newcommand{\CN}{\citeN}       %lista lunga (anno) !una cit alla volta! 
